AnomiGAN: Generative adversarial networks for anonymizing private medical data

Typical personal medical data contains sensitive information about individuals. Storing or sharing the personal medical data is thus often risky. For example, a short DNA sequence can provide information that can not only identify an individual, but also his or her relatives. Nonetheless, most countries and researchers agree on the necessity of collecting personal medical data. This stems from the fact that medical data, including genomic data, are an indispensable resource for further research and development regarding disease prevention and treatment. To prevent personal medical data from being misused, techniques to reliably preserve sensitive information should be developed for real world application. In this paper, we propose a framework called anonymized generative adversarial networks (AnomiGAN), to improve the maintenance of privacy of personal medical data, while also maintaining high prediction performance. We compared our method to state-of-the-art techniques and observed that our method preserves the same level of privacy as differential privacy (DP), but had better prediction results. We also observed that there is a trade-off between privacy and performance results depending on the degree of preservation of the original data. Here, we provide a mathematical overview of our proposed model and demonstrate its validation using UCI machine learning repository datasets in order to highlight its utility in practice. Experimentally, our approach delivers a better performance compared to that of the DP approach.

==> conclusion.tex <==
In this paper, we \textcolor{\editage}{proposed} the first DNA-steganalysis based on sequence-to-sequence learning framework using RNNs.
Our contributions can be summarized as follows:

\begin{itemize}[leftmargin=*]
    \item A new DNA-steganalysis method is proposed using RNNs.
    
    %\item Show possibility of the attack in the current DNA steganography schemes in both theoretical and practical.
        
    \item Increased robustness \textcolor{\editage}{is achieved} using unsupervised to supervised learning.
    
    %\item The improved \textcolor{\editage}{method} detects hidden messages \textcolor{\editage}{while} finding canonical/non canonical signals that \textcolor{\editage}{are} often missed by sequence analysis framework.
\end{itemize}
We \textcolor{\editage}{believe} that adopting our methodology will extend the \textcolor{\editage}{field} of DNA-steganalysis. For a future work, we plan to extend our model \textcolor{\editage}{using} automated hyperparameter tuning and \textcolor{\editage}{applying it} to diverse datasets in DNA sequences.
